Forward-fitting STIX visibilities

Aima. To determine to what extent the problem of forward fitting visibilities measured by the Spectrometer/Telescope Imaging X-rays (STIX) on-board Solar Orbiter is more challenging with respect to the same problem in the case of previous hard X-ray solar imaging missions; to identify an effective optimization scheme for parametric imaging for STIX. Methods. This paper introduces a Particle Swarm Optimization (PSO) algorithm for forward fitting STIX visibilities and compares its effectiveness with respect to the standard simplex-based optimization algorithm used so far for the analysis of visibilities measured by the Reuven Ramaty High Energy Solar Spectroscopic Imager (RHESSI). This comparison is made by considering experimental visibilities measured by both RHESSI and STIX, and synthetic visibilities generated by accounting for the STIX signal formation model. Results. We found out that the parametric imaging approach based on PSO is as reliable as the one based on the simplex method in the case of RHESSI visibilities. However, PSO is significantly more robust when applied to STIX simulated and experimental visibilities. Conclusions. Standard deterministic optimization is not effective enough for forward-fitting the few visibilities sampled by STIX in the angular frequency plane. Therefore a more sofisticated optimization scheme must be introduced for parametric imaging in the case of the Solar Orbiter X-ray telescope. The forward-fitting routine based on PSO we introduced in this paper proved to be significantly robust and reliable, and could be considered as an effective candidate tool for parametric imaging in the STIX context.

==> stralci.tex <==
\section{The STIX forward-fit problem}

\begin{figure*}[h]
\begin{center}



\tikzset{every picture/.style={line width=0.70pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.70pt,y=0.70pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,504); %set diagram left start at 0, and has height of 504

%Straight Lines [id:da8503716074860674] 
\draw    (38,180) -- (37.2,19.8) ;
\draw [shift={(37.19,16.8)}, rotate = 89.71] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da1519663475625712] 
\draw    (20,163) -- (192,163) ;
\draw [shift={(195,163)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Shape: Circle [id:dp6275471895644458] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (59,95) .. controls (59,78.43) and (72.43,65) .. (89,65) .. controls (105.57,65) and (119,78.43) .. (119,95) .. controls (119,111.57) and (105.57,125) .. (89,125) .. controls (72.43,125) and (59,111.57) .. (59,95) -- cycle ;
%Straight Lines [id:da8437642297959029] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (89,95) -- (90,162) ;
%Straight Lines [id:da4583224123100711] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (89,96) -- (36,96) ;
%Straight Lines [id:da8971340996189561] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (67,73) -- (110,117) ;
%Straight Lines [id:da6754539893746598] 
\draw    (329,180) -- (328.2,19.8) ;
\draw [shift={(328.19,16.8)}, rotate = 89.71] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da6554722478527386] 
\draw    (301,163) -- (489,163) ;
\draw [shift={(492,163)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da4177602985107105] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (380,95) -- (381,162) ;
%Straight Lines [id:da5706356014890979] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (425,95) -- (327,96) ;
%Shape: Ellipse [id:dp018778560758944796] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (336.83,114.02) .. controls (330.27,98.31) and (344.28,77.51) .. (368.12,67.55) .. controls (391.97,57.6) and (416.61,62.27) .. (423.17,77.98) .. controls (429.73,93.69) and (415.72,114.49) .. (391.88,124.45) .. controls (368.03,134.4) and (343.39,129.73) .. (336.83,114.02) -- cycle ;
%Shape: Arc [id:dp3073676640422718] 
\draw  [draw opacity=0] (400.29,87.3) .. controls (403.65,89.7) and (405.84,92.65) .. (406.59,95.92) -- (368.54,102.43) -- cycle ; \draw   (400.29,87.3) .. controls (403.65,89.7) and (405.84,92.65) .. (406.59,95.92) ;  
%Straight Lines [id:da9389573010824541] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (368.12,67.55) -- (391.88,124.45) ;
%Straight Lines [id:da7382493028664179] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (336.83,114.02) -- (423.17,77.98) ;
%Straight Lines [id:da48790976520283436] 
\draw    (394,425) -- (393.02,232) ;
\draw [shift={(393,229)}, rotate = 89.71] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da5683244642679213] 
\draw    (308,406) -- (506,405.01) ;
\draw [shift={(509,405)}, rotate = 179.71] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Shape: Circle [id:dp7854494026565917] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (415,340) .. controls (415,323.43) and (428.43,310) .. (445,310) .. controls (461.57,310) and (475,323.43) .. (475,340) .. controls (475,356.57) and (461.57,370) .. (445,370) .. controls (428.43,370) and (415,356.57) .. (415,340) -- cycle ;
%Straight Lines [id:da2106824431137173] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (445,340) -- (446,407) ;
%Straight Lines [id:da9585936114206457] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (445,341) -- (392,341) ;
%Shape: Circle [id:dp965555932212516] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (325.5,282) .. controls (325.5,269.57) and (335.57,259.5) .. (348,259.5) .. controls (360.43,259.5) and (370.5,269.57) .. (370.5,282) .. controls (370.5,294.43) and (360.43,304.5) .. (348,304.5) .. controls (335.57,304.5) and (325.5,294.43) .. (325.5,282) -- cycle ;
%Straight Lines [id:da8543778476019441] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (348,283) -- (348,410) ;
%Straight Lines [id:da7568900493601018] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (394,282) -- (348,282) ;
%Straight Lines [id:da829841114135778] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (332,268) -- (364,298) ;
%Straight Lines [id:da19790758523212215] 
\draw [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ]   (425,318) -- (465,362) ;
%Straight Lines [id:da6876965846940071] 
\draw    (39,418) -- (39,231.98) ;
\draw [shift={(39,228.98)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Straight Lines [id:da8243348544629481] 
\draw    (26,405) -- (247,405) ;
\draw [shift={(250,405)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (7.14,-3.43) -- (0,0) -- (7.14,3.43) -- cycle    ;
%Shape: Ellipse [id:dp5613757282209919] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=0.73 ] (71.04,353.59) .. controls (56.85,321.25) and (71.18,283.36) .. (103.04,268.97) .. controls (134.89,254.57) and (172.21,269.12) .. (186.4,301.46) .. controls (200.58,333.8) and (186.25,371.68) .. (154.4,386.08) .. controls (122.54,400.48) and (85.22,385.93) .. (71.04,353.59) -- cycle ;
%Shape: Ellipse [id:dp9570715025534404] 
\draw   (200.41,294.89) .. controls (203.7,302.12) and (200.09,310.92) .. (192.34,314.54) .. controls (184.6,318.17) and (175.66,315.25) .. (172.38,308.01) .. controls (169.09,300.78) and (172.71,291.98) .. (180.45,288.36) .. controls (188.19,284.73) and (197.13,287.66) .. (200.41,294.89) -- cycle ;
%Shape: Ellipse [id:dp2520636591142533] 
\draw   (191.43,283.83) .. controls (194.32,290.18) and (191.14,297.91) .. (184.34,301.09) .. controls (177.54,304.28) and (169.69,301.71) .. (166.81,295.36) .. controls (163.92,289) and (167.09,281.27) .. (173.89,278.09) .. controls (180.69,274.91) and (188.54,277.47) .. (191.43,283.83) -- cycle ;
%Shape: Ellipse [id:dp3126399393894148] 
\draw   (203.31,309.5) .. controls (206.2,315.85) and (203.02,323.58) .. (196.22,326.77) .. controls (189.43,329.95) and (181.57,327.38) .. (178.69,321.03) .. controls (175.8,314.68) and (178.98,306.95) .. (185.78,303.76) .. controls (192.58,300.58) and (200.43,303.15) .. (203.31,309.5) -- cycle ;
%Shape: Ellipse [id:dp0296229231667251] 
\draw   (182.55,274.18) .. controls (185.17,279.96) and (182.37,286.95) .. (176.29,289.79) .. controls (170.22,292.64) and (163.16,290.26) .. (160.54,284.49) .. controls (157.92,278.71) and (160.72,271.73) .. (166.79,268.88) .. controls (172.87,266.04) and (179.92,268.41) .. (182.55,274.18) -- cycle ;
%Shape: Ellipse [id:dp011250535719330657] 
\draw   (203.36,323.07) .. controls (205.98,328.84) and (203.18,335.83) .. (197.1,338.67) .. controls (191.03,341.52) and (183.98,339.14) .. (181.35,333.37) .. controls (178.73,327.6) and (181.53,320.61) .. (187.61,317.76) .. controls (193.68,314.92) and (200.73,317.29) .. (203.36,323.07) -- cycle ;
%Shape: Ellipse [id:dp4983733272554842] 
\draw   (170.71,268.6) .. controls (172.95,273.52) and (170.83,279.35) .. (165.99,281.62) .. controls (161.14,283.89) and (155.4,281.74) .. (153.16,276.82) .. controls (150.93,271.9) and (153.05,266.07) .. (157.89,263.8) .. controls (162.74,261.53) and (168.48,263.68) .. (170.71,268.6) -- cycle ;
%Shape: Ellipse [id:dp19358817347338952] 
\draw   (199.64,335.99) .. controls (201.88,340.91) and (199.76,346.74) .. (194.91,349.01) .. controls (190.07,351.28) and (184.33,349.13) .. (182.09,344.21) .. controls (179.86,339.29) and (181.97,333.46) .. (186.82,331.19) .. controls (191.67,328.92) and (197.41,331.07) .. (199.64,335.99) -- cycle ;
%Shape: Ellipse [id:dp954244938829732] 
\draw   (160.34,265.28) .. controls (162.14,269.25) and (160.43,273.94) .. (156.53,275.77) .. controls (152.63,277.59) and (148.01,275.86) .. (146.21,271.9) .. controls (144.41,267.94) and (146.11,263.24) .. (150.01,261.42) .. controls (153.92,259.59) and (158.54,261.32) .. (160.34,265.28) -- cycle ;
%Shape: Ellipse [id:dp2558701654330393] 
\draw   (195.06,345.89) .. controls (196.86,349.85) and (195.16,354.55) .. (191.26,356.37) .. controls (187.35,358.2) and (182.73,356.47) .. (180.93,352.51) .. controls (179.13,348.55) and (180.84,343.85) .. (184.74,342.03) .. controls (188.64,340.2) and (193.26,341.93) .. (195.06,345.89) -- cycle ;
%Shape: Ellipse [id:dp6318613384066838] 
\draw   (151.2,264.01) .. controls (152.54,266.97) and (151.27,270.48) .. (148.35,271.84) .. controls (145.43,273.21) and (141.98,271.91) .. (140.64,268.95) .. controls (139.29,265.99) and (140.56,262.49) .. (143.48,261.12) .. controls (146.4,259.75) and (149.85,261.05) .. (151.2,264.01) -- cycle ;
%Shape: Ellipse [id:dp5629766510652685] 
\draw   (190.1,354.14) .. controls (191.44,357.1) and (190.17,360.6) .. (187.25,361.97) .. controls (184.33,363.33) and (180.88,362.04) .. (179.53,359.08) .. controls (178.19,356.12) and (179.46,352.61) .. (182.38,351.25) .. controls (185.3,349.88) and (188.75,351.17) .. (190.1,354.14) -- cycle ;
%Straight Lines [id:da21721804433960323] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (186.4,301.45) -- (185.93,402.8) ;
%Straight Lines [id:da0001188104565443826] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (186.4,301.45) -- (38.84,301.22) ;
%Straight Lines [id:da3803898501163454] 
\draw [line width=0.75]  [dash pattern={on 0.84pt off 2.51pt}]  (145.74,221.34) -- (233.82,394.12) ;
%Curve Lines [id:da4435267527228135] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (143.48,261.12) .. controls (172.25,254.33) and (194.48,283.85) .. (200.41,294.89) ;
%Curve Lines [id:da9400657267614116] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (200.41,294.89) .. controls (208.16,317.71) and (209.02,343.76) .. (187.25,361.97) ;
%Curve Lines [id:da854619903451322] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (141.3,270.09) .. controls (158.37,281.52) and (169.68,294.27) .. (172.38,308.01) ;
%Curve Lines [id:da6738026766656409] 
\draw [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]    (172.38,308.01) .. controls (179.94,321.19) and (182.05,331.13) .. (179.08,357.74) ;
%Shape: Arc [id:dp48926067909270077] 
\draw  [draw opacity=0][line width=1.5]  (141.29,270.08) .. controls (139.57,267.94) and (139.37,264.91) .. (140.99,262.72) .. controls (142.51,260.67) and (145.18,259.97) .. (147.58,260.79) -- (145.92,266.48) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (141.29,270.08) .. controls (139.57,267.94) and (139.37,264.91) .. (140.99,262.72) .. controls (142.51,260.67) and (145.18,259.97) .. (147.58,260.79) ;  
%Shape: Arc [id:dp7407507210152406] 
\draw  [draw opacity=0][line width=1.5]  (190.11,359.07) .. controls (189.05,361.63) and (186.49,363.23) .. (183.82,362.78) .. controls (181.31,362.37) and (179.45,360.27) .. (179.07,357.71) -- (184.81,356.61) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=1.5]  (190.11,359.07) .. controls (189.05,361.63) and (186.49,363.23) .. (183.82,362.78) .. controls (181.31,362.37) and (179.45,360.27) .. (179.07,357.71) ;  
%Straight Lines [id:da021526547795055917] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (186.78,217) -- (186.4,301.45) ;
%Shape: Arc [id:dp4149112487590889] 
\draw  [draw opacity=0] (157.43,246.37) .. controls (161.65,243.87) and (166.43,242.32) .. (171.55,241.99) .. controls (177.1,241.64) and (182.43,242.76) .. (187.23,245.06) -- (173.89,279.83) -- cycle ; \draw   (157.43,246.37) .. controls (161.65,243.87) and (166.43,242.32) .. (171.55,241.99) .. controls (177.1,241.64) and (182.43,242.76) .. (187.23,245.06) ;  
%Straight Lines [id:da2741689875740272] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.75,263.88) -- (130.34,328.13) ;
%Straight Lines [id:da14245510494136204] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (130.34,328.13) -- (181.65,362.86) ;
%Curve Lines [id:da1797526238305378] 
\draw    (141.46,335.95) .. controls (141.46,332.47) and (148.3,322.05) .. (132.05,314.24) ;

% Text Node
\draw (85.37,164.72) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{c}$};
% Text Node
\draw (16.5,91.91) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$y_{c}$};
% Text Node
\draw (112,120.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\textcolor[rgb]{0.25,0.46,0.02}{f}$};
% Text Node
\draw (376.37,165.72) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{c}$};
% Text Node
\draw (305.5,90.91) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$y_{c}$};
% Text Node
\draw (353,48.9) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\textcolor[rgb]{0.25,0.46,0.02}{f}\textcolor[rgb]{0.25,0.46,0.02}{_{m}}$};
% Text Node
\draw (407.27,83.39) node [anchor=north west][inner sep=0.75pt]  [font=\small,rotate=-1.83]  {$\alpha $};
% Text Node
\draw (426.5,61.91) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\textcolor[rgb]{0.25,0.46,0.02}{f}\textcolor[rgb]{0.25,0.46,0.02}{_{M}}$};
% Text Node
\draw (442.37,410.72) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{2}$};
% Text Node
\draw (374.5,328.91) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$y_{2}$};
% Text Node
\draw (467,365.4) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\textcolor[rgb]{0.25,0.46,0.02}{f}\textcolor[rgb]{0.25,0.46,0.02}{_{2}}$};
% Text Node
\draw (396,272) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {
$
y_{1}
$};
% Text Node
\draw (341,408) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {
$
x_{1}
$};
% Text Node
\draw (314,245) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {
$
\textcolor[rgb]{0.25,0.46,0.02}{f}\textcolor[rgb]{0.25,0.46,0.02}{_{1}}
$};
% Text Node
\draw (177.17,408.29) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$x_{c}$};
% Text Node
\draw (18.23,298.85) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$y_{c}$};
% Text Node
\draw (166.68,226.97) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\alpha $};
% Text Node
\draw (143.16,311.11) node [anchor=north west][inner sep=0.75pt]  [font=\small]  {$\beta $};

\end{tikzpicture}

\end{center}

\caption{Gaussian shapes considered in the parametric imaging process.}\label{fig:fig-1}
\end{figure*}

The mathematical equation describing the image formation problem for STIX is
\begin{equation}\label{b1}
{\mathbf{V}} = {\mathbf{F}}\varphi~,
\end{equation}
where $\varphi=\varphi({\mathbf{x}})$ is the incoming photon flux emitted from location ${\mathbf{x}}=(x,y)$ on the solar disk, ${\mathbf{V}}$ is the set of $N$ visibilities measured by the telescope in correspondence of the $N$ points $\{(u_j,v_j)\}_{j=1}^{N}$ on the $(u,v)$-plane made of the 30 angular frequencies sampled by the instrument, and ${\mathbf{F}}$ is the imaging operator that maps the function representing the flaring source into samples of its Fourier transform. Mathematically,
\begin{equation}\label{b2}
({\bf{F}}\varphi)_j = \int\int dx dy \varphi(x,y) e^{i2\pi(u_j x + v_j y)}~~~j=1,\ldots,30~.
\end{equation}
Therefore, the STIX imaging problem is the one of reconstructing the photon flux $\varphi$ from experimental representatives of ${\mathbf{V}}$. This problem is linear but does not have a unique solution, due to the notably sparse sampling of the data space.

Imaging procedures based on forward fitting estimate the parameters of parametric shapes of the flaring source. Physical considerations about hard X-rays emission and the experience gained during the RHESSI mission suggest that appropriate parametric shapes are:
\begin{itemize}
\item A Gaussian circular source ({\em{single}} from now on) centered at $(x_{c}, y_{c})$
\begin{equation}
\varphi_C(x,y) = \frac{\phi}{2 \pi \sigma^2} \exp\left(- \frac{(x-x_c)^2 + (y-y_c)^2}{2\sigma^2} \right)~,
\end{equation}
where $\phi$ is the total flux of the source, $\sigma = FWHM / \left(2 \sqrt{2 \log 2}\right)$ and $FWHM$ is the Full Width at Half Maximum of the source. The set of parameters for this source is ${ \boldsymbol{\theta}}_C = (\phi, FWHM, x_{c}, y_{c})$.
\item A Gaussian elliptical source ({\em{ellipse}} from now on) centered at $(x_{c}, y_{c})$
\begin{equation}
\varphi_E(x,y) = \frac{\phi}{2 \pi \sigma_M \sigma_m} \exp\left(-\frac{x'^2}{2 \sigma_M^2} - \frac{y'^2}{2\sigma_m^2} \right)~,
\end{equation}
where $\phi$ is the total flux of the source, $\sigma_M = FWHM_M / \left(2 \sqrt{2 \log 2}\right)$, $\sigma_m = FWHM_m / \left(2 \sqrt{2 \log 2}\right)$, $FWHM_M$ is the major FWHM and $FWHM_m$ is the minor FWHM. Further,
\begin{equation}
x' = \cos(\alpha) (x-x_{c}) + \sin(\alpha) (y-y_{c})
\end{equation}
\begin{equation}
y' = -\sin(\alpha) (x-x_{c}) + \cos(\alpha) (y-y_{c})
\end{equation}
where $\alpha$ is the angle between the semi-major and the $x$-axis measured counterclockwise. The set of parameters for the elliptical source is ${ \boldsymbol{\theta}}_E = (\phi, FWHM_M, FWHM_m, \alpha, x_c, y_c)$ 
%\footnote{We point out that we actually optimize the two auxiliary variables: $\varepsilon \in (0,1)$ and $f$, satisfying  $f_M = f \; (1-\varepsilon^2)^{-\frac{1}{4}}$ and $f_m = f \;  (1-\varepsilon^2)^{\frac{1}{4}}$.}.%, and so ${\bf \boldsymbol{\theta}}_E = (\phi, \varepsilon, f, \alpha)$.}.
\item A double Gaussian circular source ({\em{double}} from now on), one source centered at $(x_{1}, y_{1})$ and the second one at $(x_{2}, y_{2})$,
\begin{equation}
\begin{array}{ll}
\varphi_D(x,y) & =  \frac{\phi_1}{2 \pi \sigma_1^2} \exp\left(-\frac{(x - x_1)^2 + (y - y_1)^2}{2\sigma_1^2} \right) \\ 
& +   \frac{\phi_2}{2 \pi \sigma_2^2} \exp\left(-\frac{(x - x_2)^2 + (y - y_2)^2}{2\sigma_2^2} \right) ~,\\
\end{array}
\end{equation}
where $\phi_j$ is the total flux, $\sigma_j = FWHM_j / \left(2 \sqrt{2 \log 2}\right)$ and $FWHM_j$ is the FWHM ($j=1,2$). The set of parameters for the double circular source is ${ \boldsymbol{\theta}}_D = (\phi_1, FWHM_1, \phi_2, FWHM_2, x_1, y_1, x_2, y_2)$.
\item The replication of 21 singles with centers located along a circle to represent a thermal loop ({\em{loop}} from now on).
\end{itemize}
The shapes of the four parametric sources are illustrated in Figure \ref{fig:fig-1}. 

We denote as ${ \boldsymbol{\theta}}$ the set of parameters characterizing each source shape. Then, forward-fitting STIX visibilities for parametric imaging requires the solution of the optimization problem 
\begin{equation}\label{min-prob}
\argmin_{{ \boldsymbol{\theta}}\in {\cal D}} \hskip 0.2cm \chi^2({ \boldsymbol{\theta}}), 
\end{equation}
where ${\cal D}$ is the so-called feasibility region for the imaging parameter ${ \boldsymbol{\theta}}$. The target function $\chi^2({ \boldsymbol{\theta}})$ is defined as
\begin{equation}\label{chi2}
\chi^2({ \boldsymbol{\theta}}) = \frac{1}{30-N_{{ \boldsymbol{\theta}}}} \sum_{i=1}^{24} \left |  \frac{V_{i}^{exp} - V_{i}^{pr}({ \boldsymbol{\theta}})}{\sigma_i}   \right |^2 \ ,
\end{equation}
where $N_{{ \boldsymbol{\theta}}}$ is the number of parameters of the source shape function, $V_{i}^{exp}$ is the $i$-th visibility measured by STIX, $V_{i}^{pr}({ \boldsymbol{\theta}})$ is the $i$-th visibility predicted by the parametric source function, and $\sigma_i$ is the uncertainty on the $i-$th measured visibility amplitude. 

The parametric imaging problem for STIX consists in selecting a specific shape function as candidate source, solving problem (\ref{min-prob})-(\ref{chi2}), and feeding the corresponding source shape with the solution parameters. The computational core of this procedure is the optimization scheme applied for solving (\ref{min-prob})-(\ref{chi2}). In the Solar SoftWare (SSW) repository the VIS$\_$FWDFIT routine utilizes the simplex scheme (AMOEBA) and has been applied for the parametric imaging of all RHESSI data sets published so far. The effectiveness of this approach significantly decreases when the number of data at disposal becomes smaller, as is the case of STIX measurements. Therefore, in this framework, new optimization approaches must be introduced, which are able to avoid local minima by means of a more effective exploration of the parameter space.

\section{Particle Swarm Optimization}
Particle Swarm Optimization (PSO) \citep{eberhart1995particle,Qasem} realizes optimization by mimicking swarm intelligence. The starting point of swarm intelligence is to populate the parameter space $\Theta$ by means of a cloud of points named {\em{cloud}} and {\em{birds}}, respectively, and its goal is to mimic the trajectory of each bird by numerically implementing the fact that the target of a flock is to search for the maximum availability of food. This is done by assuming that
\begin{itemize}
    \item The maximum availability of food corresponds to the minimum of the objective function \ref{chi2}.
    \item When a bird visits a local minimum, then the other birds can either move away from flock toward the minimum ({\em{selfish behavior}}) or stay close to the flock ({\em{social behavior}}).
\end{itemize}
As a result, if the two behaviors are well-balanced, the flock of birds gradually approaches the global minimum.

The IDL PSO routine we have implemented and included in SSW is based on the implementation introduced by (reference: Coello). Differently than for VIS$\_$FWDFIT, VIS$\_$FWDFIT$\_$PSO has been implemented in such a way that the user can decide which parameters have to be optimized while keeping the other ones fixed. In VIS$\_$FWDFIT$\_$PSO uncertainty quantification is computed by generating a confidence strip on each parameter value: several realizations of the input data are computed by randomly perturbing the experimental set of visibility amplitudes with Gaussian noise whose standard deviation is set equal to the errors on the measurements; for each realization VIS$\_$FWDFIT$\_$PSO is applied; and, finally, the standard deviation of each optimized source parameter is computed.
